Parallel Integration over Simple Radical Extensions in Mixed Towers: Charlwood's Integrals

We evaluate a SymPy implementation of the parallel Risch-Norman method using Charlwood's 2008 suite of 50 challenging indefinite integrals. The system automatically builds integrand towers, verifies answers by differentiation, and returns correct, verified integrals for 49 problems with zero errors. The single failure, $\int\arcsin(x\sqrt{1-x^2})\,dx$, is proven non-elementary using a holomorphic-remainder certificate, though limited by an unverified completeness hypothesis on a genus-three curve. Part II's degree bounds successfully reduce classical ansatz sizes by two-thirds without impacting running time. The paper details algorithmic mechanisms like $S'$-units, Pell units, and residue computing in tower coordinates. Compared to mature implementations, this untuned SymPy prototype is slower than FriCAS (by a factor of six on the median integral) but more accurate than AXIOM (which returned three wrong answers). Profiling pinpoints performance bottlenecks in nonlinear norm searches and nested number fields, outlining clear targets for optimisation.

==> charlwood_numbers.tex <==
% generated by charlwood_report.py
\makeatletter
\expandafter\def\csname tpm@P1\endcsname{0.5}
\expandafter\def\csname tfr@P1\endcsname{0.1}
\expandafter\def\csname tax@P1\endcsname{0.2}
\expandafter\def\csname spm@P1\endcsname{\checkmark}
\expandafter\def\csname sfr@P1\endcsname{\checkmark}
\expandafter\def\csname sax@P1\endcsname{\checkmark}
\expandafter\def\csname tpm@P2\endcsname{0.2}
\expandafter\def\csname tfr@P2\endcsname{0.1}
\expandafter\def\csname tax@P2\endcsname{0.1}
\expandafter\def\csname spm@P2\endcsname{\checkmark}
\expandafter\def\csname sfr@P2\endcsname{\checkmark}
\expandafter\def\csname sax@P2\endcsname{\checkmark}
\expandafter\def\csname tpm@P3\endcsname{2.0}
\expandafter\def\csname tfr@P3\endcsname{52.8}
\expandafter\def\csname tax@P3\endcsname{--}
\expandafter\def\csname spm@P3\endcsname{\checkmark}
\expandafter\def\csname sfr@P3\endcsname{\checkmark}
\expandafter\def\csname sax@P3\endcsname{\textsf{E}}
\expandafter\def\csname tpm@P4\endcsname{6.2}
\expandafter\def\csname tfr@P4\endcsname{0.1}
\expandafter\def\csname tax@P4\endcsname{0.1}
\expandafter\def\csname spm@P4\endcsname{\checkmark}
\expandafter\def\csname sfr@P4\endcsname{\checkmark}
\expandafter\def\csname sax@P4\endcsname{\checkmark}
\expandafter\def\csname tpm@P5\endcsname{2.6}
\expandafter\def\csname tfr@P5\endcsname{0.2}
\expandafter\def\csname tax@P5\endcsname{0.5}
\expandafter\def\csname spm@P5\endcsname{\checkmark}
\expandafter\def\csname sfr@P5\endcsname{\checkmark}
\expandafter\def\csname sax@P5\endcsname{\checkmark}
\expandafter\def\csname tpm@P6\endcsname{0.6}
\expandafter\def\csname tfr@P6\endcsname{0.2}
\expandafter\def\csname tax@P6\endcsname{0.5}
\expandafter\def\csname spm@P6\endcsname{\checkmark}
\expandafter\def\csname sfr@P6\endcsname{\checkmark}
\expandafter\def\csname sax@P6\endcsname{\checkmark}
\expandafter\def\csname tpm@P7\endcsname{0.2}
\expandafter\def\csname tfr@P7\endcsname{0.2}
\expandafter\def\csname tax@P7\endcsname{0.4}
\expandafter\def\csname spm@P7\endcsname{\checkmark}
\expandafter\def\csname sfr@P7\endcsname{\checkmark}
\expandafter\def\csname sax@P7\endcsname{\checkmark}
\expandafter\def\csname tpm@P8\endcsname{7.0}
\expandafter\def\csname tfr@P8\endcsname{0.7}
\expandafter\def\csname tax@P8\endcsname{12.2}
\expandafter\def\csname spm@P8\endcsname{\checkmark}
\expandafter\def\csname sfr@P8\endcsname{\checkmark}
\expandafter\def\csname sax@P8\endcsname{\checkmark}
\expandafter\def\csname tpm@P9\endcsname{0.5}
\expandafter\def\csname tfr@P9\endcsname{0.1}
\expandafter\def\csname tax@P9\endcsname{--}
\expandafter\def\csname spm@P9\endcsname{\checkmark}
\expandafter\def\csname sfr@P9\endcsname{\checkmark}
\expandafter\def\csname sax@P9\endcsname{\textsf{E}}
\expandafter\def\csname tpm@P10\endcsname{0.5}
\expandafter\def\csname tfr@P10\endcsname{0.1}
\expandafter\def\csname tax@P10\endcsname{0.1}
\expandafter\def\csname spm@P10\endcsname{\checkmark}
\expandafter\def\csname sfr@P10\endcsname{\checkmark}
\expandafter\def\csname sax@P10\endcsname{\checkmark}
\expandafter\def\csname tpm@A1\endcsname{1.3}
\expandafter\def\csname tfr@A1\endcsname{0.1}
\expandafter\def\csname tax@A1\endcsname{0.1}
\expandafter\def\csname spm@A1\endcsname{\checkmark}
\expandafter\def\csname sfr@A1\endcsname{\checkmark}
\expandafter\def\csname sax@A1\endcsname{\checkmark}
\expandafter\def\csname tpm@A2\endcsname{3.6}
\expandafter\def\csname tfr@A2\endcsname{0.1}
\expandafter\def\csname tax@A2\endcsname{0.2}
\expandafter\def\csname spm@A2\endcsname{\checkmark}
\expandafter\def\csname sfr@A2\endcsname{\checkmark}
\expandafter\def\csname sax@A2\endcsname{\textsf{W}}
\expandafter\def\csname tpm@A3\endcsname{3.1}
\expandafter\def\csname tfr@A3\endcsname{0.1}
\expandafter\def\csname tax@A3\endcsname{0.2}
\expandafter\def\csname spm@A3\endcsname{\checkmark}
\expandafter\def\csname sfr@A3\endcsname{\checkmark}
\expandafter\def\csname sax@A3\endcsname{\textsf{W}}
\expandafter\def\csname tpm@A4\endcsname{0.7}
\expandafter\def\csname tfr@A4\endcsname{0.1}
\expandafter\def\csname tax@A4\endcsname{0.1}
\expandafter\def\csname spm@A4\endcsname{\checkmark}
\expandafter\def\csname sfr@A4\endcsname{\checkmark}
\expandafter\def\csname sax@A4\endcsname{\checkmark}
\expandafter\def\csname tpm@A5\endcsname{1.1}
\expandafter\def\csname tfr@A5\endcsname{0.1}
\expandafter\def\csname tax@A5\endcsname{--}
\expandafter\def\csname spm@A5\endcsname{\checkmark}
\expandafter\def\csname sfr@A5\endcsname{\checkmark}
\expandafter\def\csname sax@A5\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A6\endcsname{1.7}
\expandafter\def\csname tfr@A6\endcsname{0.1}
\expandafter\def\csname tax@A6\endcsname{--}
\expandafter\def\csname spm@A6\endcsname{\checkmark}
\expandafter\def\csname sfr@A6\endcsname{\checkmark}
\expandafter\def\csname sax@A6\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A7\endcsname{1.1}
\expandafter\def\csname tfr@A7\endcsname{0.1}
\expandafter\def\csname tax@A7\endcsname{--}
\expandafter\def\csname spm@A7\endcsname{\checkmark}
\expandafter\def\csname sfr@A7\endcsname{\checkmark}
\expandafter\def\csname sax@A7\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A8\endcsname{0.3}
\expandafter\def\csname tfr@A8\endcsname{0.1}
\expandafter\def\csname tax@A8\endcsname{0.1}
\expandafter\def\csname spm@A8\endcsname{\checkmark}
\expandafter\def\csname sfr@A8\endcsname{\checkmark}
\expandafter\def\csname sax@A8\endcsname{\checkmark}
\expandafter\def\csname tpm@A9\endcsname{0.2}
\expandafter\def\csname tfr@A9\endcsname{0.1}
\expandafter\def\csname tax@A9\endcsname{0.1}
\expandafter\def\csname spm@A9\endcsname{\checkmark}
\expandafter\def\csname sfr@A9\endcsname{\checkmark}
\expandafter\def\csname sax@A9\endcsname{\checkmark}
\expandafter\def\csname tpm@A10\endcsname{0.1}
\expandafter\def\csname tfr@A10\endcsname{0.1}
\expandafter\def\csname tax@A10\endcsname{0.1}
\expandafter\def\csname spm@A10\endcsname{\checkmark}
\expandafter\def\csname sfr@A10\endcsname{\checkmark}
\expandafter\def\csname sax@A10\endcsname{\checkmark}
\expandafter\def\csname tpm@A11\endcsname{1.3}
\expandafter\def\csname tfr@A11\endcsname{0.1}
\expandafter\def\csname tax@A11\endcsname{--}
\expandafter\def\csname spm@A11\endcsname{\checkmark}
\expandafter\def\csname sfr@A11\endcsname{\checkmark}
\expandafter\def\csname sax@A11\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A12\endcsname{1.6}
\expandafter\def\csname tfr@A12\endcsname{0.1}
\expandafter\def\csname tax@A12\endcsname{--}
\expandafter\def\csname spm@A12\endcsname{\checkmark}
\expandafter\def\csname sfr@A12\endcsname{\checkmark}
\expandafter\def\csname sax@A12\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A13\endcsname{0.4}
\expandafter\def\csname tfr@A13\endcsname{0.1}
\expandafter\def\csname tax@A13\endcsname{0.1}
\expandafter\def\csname spm@A13\endcsname{\checkmark}
\expandafter\def\csname sfr@A13\endcsname{\checkmark}
\expandafter\def\csname sax@A13\endcsname{\checkmark}
\expandafter\def\csname tpm@A14\endcsname{0.3}
\expandafter\def\csname tfr@A14\endcsname{0.1}
\expandafter\def\csname tax@A14\endcsname{0.1}
\expandafter\def\csname spm@A14\endcsname{\checkmark}
\expandafter\def\csname sfr@A14\endcsname{\checkmark}
\expandafter\def\csname sax@A14\endcsname{\checkmark}
\expandafter\def\csname tpm@A15\endcsname{0.1}
\expandafter\def\csname tfr@A15\endcsname{0.1}
\expandafter\def\csname tax@A15\endcsname{0.1}
\expandafter\def\csname spm@A15\endcsname{\checkmark}
\expandafter\def\csname sfr@A15\endcsname{\checkmark}
\expandafter\def\csname sax@A15\endcsname{\checkmark}
\expandafter\def\csname tpm@A16\endcsname{1.4}
\expandafter\def\csname tfr@A16\endcsname{0.1}
\expandafter\def\csname tax@A16\endcsname{0.1}
\expandafter\def\csname spm@A16\endcsname{\checkmark}
\expandafter\def\csname sfr@A16\endcsname{\checkmark}
\expandafter\def\csname sax@A16\endcsname{\checkmark}
\expandafter\def\csname tpm@A17\endcsname{0.3}
\expandafter\def\csname tfr@A17\endcsname{0.1}
\expandafter\def\csname tax@A17\endcsname{0.1}
\expandafter\def\csname spm@A17\endcsname{\checkmark}
\expandafter\def\csname sfr@A17\endcsname{\checkmark}
\expandafter\def\csname sax@A17\endcsname{\checkmark}
\expandafter\def\csname tpm@A18\endcsname{0.2}
\expandafter\def\csname tfr@A18\endcsname{0.1}
\expandafter\def\csname tax@A18\endcsname{0.1}
\expandafter\def\csname spm@A18\endcsname{\checkmark}
\expandafter\def\csname sfr@A18\endcsname{\checkmark}
\expandafter\def\csname sax@A18\endcsname{\checkmark}
\expandafter\def\csname tpm@A19\endcsname{1.1}
\expandafter\def\csname tfr@A19\endcsname{0.1}
\expandafter\def\csname tax@A19\endcsname{0.2}
\expandafter\def\csname spm@A19\endcsname{\checkmark}
\expandafter\def\csname sfr@A19\endcsname{\checkmark}
\expandafter\def\csname sax@A19\endcsname{\checkmark}
\expandafter\def\csname tpm@A20\endcsname{0.6}
\expandafter\def\csname tfr@A20\endcsname{0.1}
\expandafter\def\csname tax@A20\endcsname{0.1}
\expandafter\def\csname spm@A20\endcsname{\checkmark}
\expandafter\def\csname sfr@A20\endcsname{\checkmark}
\expandafter\def\csname sax@A20\endcsname{\checkmark}
\expandafter\def\csname tpm@A21\endcsname{0.7}
\expandafter\def\csname tfr@A21\endcsname{0.1}
\expandafter\def\csname tax@A21\endcsname{0.2}
\expandafter\def\csname spm@A21\endcsname{\checkmark}
\expandafter\def\csname sfr@A21\endcsname{\checkmark}
\expandafter\def\csname sax@A21\endcsname{\checkmark}
\expandafter\def\csname tpm@A22\endcsname{0.4}
\expandafter\def\csname tfr@A22\endcsname{0.1}
\expandafter\def\csname tax@A22\endcsname{0.1}
\expandafter\def\csname spm@A22\endcsname{\checkmark}
\expandafter\def\csname sfr@A22\endcsname{\checkmark}
\expandafter\def\csname sax@A22\endcsname{\checkmark}
\expandafter\def\csname tpm@A23\endcsname{0.3}
\expandafter\def\csname tfr@A23\endcsname{0.1}
\expandafter\def\csname tax@A23\endcsname{0.1}
\expandafter\def\csname spm@A23\endcsname{\checkmark}
\expandafter\def\csname sfr@A23\endcsname{\checkmark}
\expandafter\def\csname sax@A23\endcsname{\checkmark}
\expandafter\def\csname tpm@A24\endcsname{0.2}
\expandafter\def\csname tfr@A24\endcsname{0.1}
\expandafter\def\csname tax@A24\endcsname{0.1}
\expandafter\def\csname spm@A24\endcsname{\checkmark}
\expandafter\def\csname sfr@A24\endcsname{\checkmark}
\expandafter\def\csname sax@A24\endcsname{\checkmark}
\expandafter\def\csname tpm@A25\endcsname{0.3}
\expandafter\def\csname tfr@A25\endcsname{0.1}
\expandafter\def\csname tax@A25\endcsname{--}
\expandafter\def\csname spm@A25\endcsname{\checkmark}
\expandafter\def\csname sfr@A25\endcsname{\checkmark}
\expandafter\def\csname sax@A25\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A26\endcsname{0.2}
\expandafter\def\csname tfr@A26\endcsname{0.1}
\expandafter\def\csname tax@A26\endcsname{0.1}
\expandafter\def\csname spm@A26\endcsname{\checkmark}
\expandafter\def\csname sfr@A26\endcsname{\checkmark}
\expandafter\def\csname sax@A26\endcsname{\checkmark}
\expandafter\def\csname tpm@A27\endcsname{4.2}
\expandafter\def\csname tfr@A27\endcsname{0.1}
\expandafter\def\csname tax@A27\endcsname{--}
\expandafter\def\csname spm@A27\endcsname{\checkmark}
\expandafter\def\csname sfr@A27\endcsname{\checkmark}
\expandafter\def\csname sax@A27\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A28\endcsname{3.7}
\expandafter\def\csname tfr@A28\endcsname{0.1}
\expandafter\def\csname tax@A28\endcsname{0.1}
\expandafter\def\csname spm@A28\endcsname{\checkmark}
\expandafter\def\csname sfr@A28\endcsname{\checkmark}
\expandafter\def\csname sax@A28\endcsname{\checkmark}
\expandafter\def\csname tpm@A29\endcsname{2.9}
\expandafter\def\csname tfr@A29\endcsname{0.1}
\expandafter\def\csname tax@A29\endcsname{0.1}
\expandafter\def\csname spm@A29\endcsname{\checkmark}
\expandafter\def\csname sfr@A29\endcsname{\checkmark}
\expandafter\def\csname sax@A29\endcsname{\checkmark}
\expandafter\def\csname tpm@A30\endcsname{0.5}
\expandafter\def\csname tfr@A30\endcsname{0.1}
\expandafter\def\csname tax@A30\endcsname{0.2}
\expandafter\def\csname spm@A30\endcsname{\checkmark}
\expandafter\def\csname sfr@A30\endcsname{\checkmark}
\expandafter\def\csname sax@A30\endcsname{\checkmark}
\expandafter\def\csname tpm@A31\endcsname{0.9}
\expandafter\def\csname tfr@A31\endcsname{0.1}
\expandafter\def\csname tax@A31\endcsname{--}
\expandafter\def\csname spm@A31\endcsname{\checkmark}
\expandafter\def\csname sfr@A31\endcsname{\checkmark}
\expandafter\def\csname sax@A31\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A32\endcsname{0.6}
\expandafter\def\csname tfr@A32\endcsname{0.2}
\expandafter\def\csname tax@A32\endcsname{0.2}
\expandafter\def\csname spm@A32\endcsname{\checkmark}
\expandafter\def\csname sfr@A32\endcsname{\checkmark}
\expandafter\def\csname sax@A32\endcsname{\textsf{W}}
\expandafter\def\csname tpm@A33\endcsname{0.5}
\expandafter\def\csname tfr@A33\endcsname{0.1}
\expandafter\def\csname tax@A33\endcsname{0.4}
\expandafter\def\csname spm@A33\endcsname{\checkmark}
\expandafter\def\csname sfr@A33\endcsname{\checkmark}
\expandafter\def\csname sax@A33\endcsname{\checkmark}
\expandafter\def\csname tpm@A34\endcsname{0.7}
\expandafter\def\csname tfr@A34\endcsname{0.2}
\expandafter\def\csname tax@A34\endcsname{0.3}
\expandafter\def\csname spm@A34\endcsname{\checkmark}
\expandafter\def\csname sfr@A34\endcsname{\checkmark}
\expandafter\def\csname sax@A34\endcsname{\checkmark}
\expandafter\def\csname tpm@A35\endcsname{4.1}
\expandafter\def\csname tfr@A35\endcsname{7.7}
\expandafter\def\csname tax@A35\endcsname{--}
\expandafter\def\csname spm@A35\endcsname{\checkmark}
\expandafter\def\csname sfr@A35\endcsname{\checkmark}
\expandafter\def\csname sax@A35\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A36\endcsname{0.1}
\expandafter\def\csname tfr@A36\endcsname{0.1}
\expandafter\def\csname tax@A36\endcsname{0.1}
\expandafter\def\csname spm@A36\endcsname{\checkmark}
\expandafter\def\csname sfr@A36\endcsname{\checkmark}
\expandafter\def\csname sax@A36\endcsname{\checkmark}
\expandafter\def\csname tpm@A37\endcsname{2.1}
\expandafter\def\csname tfr@A37\endcsname{0.1}
\expandafter\def\csname tax@A37\endcsname{0.1}
\expandafter\def\csname spm@A37\endcsname{\checkmark}
\expandafter\def\csname sfr@A37\endcsname{\checkmark}
\expandafter\def\csname sax@A37\endcsname{\checkmark}
\expandafter\def\csname tpm@A38\endcsname{0.4}
\expandafter\def\csname tfr@A38\endcsname{0.1}
\expandafter\def\csname tax@A38\endcsname{0.1}
\expandafter\def\csname spm@A38\endcsname{\checkmark}
\expandafter\def\csname sfr@A38\endcsname{\checkmark}
\expandafter\def\csname sax@A38\endcsname{\checkmark}
\expandafter\def\csname tpm@A39\endcsname{1.6}
\expandafter\def\csname tfr@A39\endcsname{0.1}
\expandafter\def\csname tax@A39\endcsname{--}
\expandafter\def\csname spm@A39\endcsname{\textsf{F}}
\expandafter\def\csname sfr@A39\endcsname{\textsf{U}}
\expandafter\def\csname sax@A39\endcsname{\textsf{E}}
\expandafter\def\csname tpm@A40\endcsname{2.8}
\expandafter\def\csname tfr@A40\endcsname{0.2}
\expandafter\def\csname tax@A40\endcsname{0.2}
\expandafter\def\csname spm@A40\endcsname{\checkmark}
\expandafter\def\csname sfr@A40\endcsname{\checkmark}
\expandafter\def\csname sax@A40\endcsname{\checkmark}
\expandafter\def\csname tsf@A16\endcsname{2.1}
\expandafter\def\csname tsf@A1\endcsname{1.1}
\expandafter\def\csname tsf@A2\endcsname{10.6}
\expandafter\def\csname tsf@A3\endcsname{10.4}
\expandafter\def\csname tsf@P4\endcsname{23.9}
\expandafter\def\csname wax@P1\endcsname{0.9}
\expandafter\def\csname wax@P2\endcsname{0.9}
\expandafter\def\csname wax@P3\endcsname{173.7}
\expandafter\def\csname wax@P4\endcsname{1.0}
\expandafter\def\csname wax@P5\endcsname{1.4}
\expandafter\def\csname wax@P6\endcsname{1.4}
\expandafter\def\csname wax@P7\endcsname{1.3}
\expandafter\def\csname wax@P8\endcsname{14.6}
\expandafter\def\csname wax@P9\endcsname{1.1}
\expandafter\def\csname wax@P10\endcsname{1.1}
\expandafter\def\csname wax@A1\endcsname{1.1}
\expandafter\def\csname wax@A2\endcsname{1.2}
\expandafter\def\csname wax@A3\endcsname{1.3}
\expandafter\def\csname wax@A4\endcsname{1.1}
\expandafter\def\csname wax@A5\endcsname{1.1}
\expandafter\def\csname wax@A6\endcsname{1.3}
\expandafter\def\csname wax@A7\endcsname{1.1}
\expandafter\def\csname wax@A8\endcsname{1.0}
\expandafter\def\csname wax@A9\endcsname{1.0}
\expandafter\def\csname wax@A10\endcsname{1.0}
\expandafter\def\csname wax@A11\endcsname{1.6}
\expandafter\def\csname wax@A12\endcsname{1.5}
\expandafter\def\csname wax@A13\endcsname{1.1}
\expandafter\def\csname wax@A14\endcsname{1.0}
\expandafter\def\csname wax@A15\endcsname{1.0}
\expandafter\def\csname wax@A16\endcsname{1.4}
\expandafter\def\csname wax@A17\endcsname{1.0}
\expandafter\def\csname wax@A18\endcsname{1.1}
\expandafter\def\csname wax@A19\endcsname{1.2}
\expandafter\def\csname wax@A20\endcsname{1.1}
\expandafter\def\csname wax@A21\endcsname{1.2}
\expandafter\def\csname wax@A22\endcsname{1.1}
\expandafter\def\csname wax@A23\endcsname{1.1}
\expandafter\def\csname wax@A24\endcsname{1.0}
\expandafter\def\csname wax@A25\endcsname{1.7}
\expandafter\def\csname wax@A26\endcsname{1.1}
\expandafter\def\csname wax@A27\endcsname{1.0}
\expandafter\def\csname wax@A28\endcsname{1.1}
\expandafter\def\csname wax@A29\endcsname{1.1}
\expandafter\def\csname wax@A30\endcsname{1.3}
\expandafter\def\csname wax@A31\endcsname{1.0}
\expandafter\def\csname wax@A32\endcsname{1.2}
\expandafter\def\csname wax@A33\endcsname{1.5}
\expandafter\def\csname wax@A34\endcsname{1.3}
\expandafter\def\csname wax@A35\endcsname{43.8}
\expandafter\def\csname wax@A36\endcsname{1.0}
\expandafter\def\csname wax@A37\endcsname{1.1}
\expandafter\def\csname wax@A38\endcsname{1.0}
\expandafter\def\csname wax@A39\endcsname{1.4}
\expandafter\def\csname wax@A40\endcsname{1.1}
\newcommand{\tpm}[1]{\csname tpm@#1\endcsname}
\newcommand{\tfr}[1]{\csname tfr@#1\endcsname}
\newcommand{\tax}[1]{\csname tax@#1\endcsname}
\newcommand{\spm}[1]{\csname spm@#1\endcsname}
\newcommand{\sfr}[1]{\csname sfr@#1\endcsname}
\newcommand{\sax}[1]{\csname sax@#1\endcsname}
\newcommand{\tsf}[1]{\csname tsf@#1\endcsname}
\newcommand{\wax}[1]{\csname wax@#1\endcsname}
\newcommand{\npm}{49}
\newcommand{\nfr}{49}
\newcommand{\nax}{35}
\newcommand{\totpm}{68}
\newcommand{\meanpm}{1.4}
\newcommand{\medpm}{0.6}
\newcommand{\totfr}{67}
\newcommand{\meanfr}{1.3}
\newcommand{\medfr}{0.1}
\newcommand{\totax}{18}
\newcommand{\meanax}{0.5}
\newcommand{\medax}{0.1}
\makeatother

